Geranos: a Novel Tilted-Rotors Aerial Robot for the Transportation of Poles

In challenging terrains, constructing structures such as antennas and cable-car masts often requires the use of helicopters to transport loads via ropes. The swinging of the load, exacerbated by wind, impairs positioning accuracy, therefore necessitating precise manual placement by ground crews. This increases costs and risk of injuries. Challenging this paradigm, we present Geranos: a specialized multirotor Unmanned Aerial Vehicle (UAV) designed to enhance aerial transportation and assembly. Geranos demonstrates exceptional prowess in accurately positioning vertical poles, achieving this through an innovative integration of load transport and precision. Its unique ring design mitigates the impact of high pole inertia, while a lightweight two-part grasping mechanism ensures secure load attachment without active force. With four primary propellers countering gravity and four auxiliary ones enhancing lateral precision, Geranos achieves comprehensive position and attitude control around hovering. Our experimental demonstration mimicking antenna/cable-car mast installations showcases Geranos ability in stacking poles (3 kg, 2 m long) with remarkable sub-5 cm placement accuracy, without the need of human manual intervention.

==> cover_letter.tex <==

% Cover letter

 

% The authors will have to explicitly declare in the cover letter, if their article aims to be considered for publication as Reproducible Article (R-Article), as a short article illustrating the replication of other authors’ results (a ‘r-article’), or a short reply by the authors of a reproduced experiment.

 

% It is the responsibility of the authors to publish all the necessary information to make their results reproducible.




Cover letter:

Dear editor,

We are pleased to submit our work entitled 'Geranos: a Novel Tilted-Rotors Aerial Robot for the Transportation of Poles' to be considered for publication in the IEEE Robotics & Automation Magazine. 
The work has not been published or submitted simultaneously for publication elsewhere.

In this work, we present a newly developed tilted-rotors aerial robot Geranos, which is capable of transporting poles of up to three kilograms of mass and three meters of length. It's unique propeller setup and grabbing mechanism help it to be a simple, lightweight and precise solution for this exact problem. In a flight demonstration we show the capabilities of Geranos by stacking two one meter long poles on top of each other.

We are convinced that our work could be very useful for many colleagues as well as industry and that the IEEE Robotics & Automation Magazine as a journal is the ideal venue to introduce it.

In the name of all authors, thank you for considering our work for review. We highly appreciate your time and we are looking forward to your response.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

